To Softmax, or not to Softmax: that is the question when applying Active Learning for Transformer Models

Despite achieving state-of-the-art results in nearly all Natural Language Processing applications, fine-tuning Transformer-based language models still requires a significant amount of labeled data to work. A well known technique to reduce the amount of human effort in acquiring a labeled dataset is \textit{Active Learning} (AL): an iterative process in which only the minimal amount of samples is labeled. AL strategies require access to a quantified confidence measure of the model predictions. A common choice is the softmax activation function for the final layer. As the softmax function provides misleading probabilities, this paper compares eight alternatives on seven datasets. Our almost paradoxical finding is that most of the methods are too good at identifying the true most uncertain samples (outliers), and that labeling therefore exclusively outliers results in worse performance. As a heuristic we propose to systematically ignore samples, which results in improvements of various methods compared to the softmax function.

==> BTW To softmax, or not to softmax that is the question (Arxiv Version) (1)/figures/merge_datasets_test_acc__baseline_bert-base-uncased_5_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT              & IM              & CL              & S2              &   Mean \\
\midrule
 KLD 95   & 75.10 +- (8.74) & 76.06 +- (6.00) & 87.09 +- (5.62) & 73.30 +- (8.38) & 69.30 +- (3.09) & 71.97 +- (1.22) & 81.31 +- (5.49) &  76.30 \\
 Ent 95   & 90.89 +- (1.84) & 87.17 +- (0.98) & 86.61 +- (6.55) & 72.75 +- (5.02) & 66.27 +- (4.57) & 72.19 +- (1.06) & 73.85 +- (5.96) &  78.53 \\
 VE 95    & 89.34 +- (2.18) & 87.39 +- (0.59) & 94.10 +- (0.55) & 74.41 +- (4.48) & 57.93 +- (9.43) & 71.75 +- (0.97) & 79.39 +- (6.50) &  79.19 \\
 TeSc 95  & 92.94 +- (0.60) & 88.67 +- (0.48) & 95.41 +- (0.27) & 78.88 +- (1.59) & 69.99 +- (2.61) & 74.76 +- (2.39) & 86.11 +- (1.63) &  83.82 \\
 IS 95    & 93.31 +- (0.82) & 88.70 +- (0.33) & 95.45 +- (0.31) & 78.03 +- (3.15) & 70.48 +- (1.82) & 75.01 +- (1.93) & 86.01 +- (1.56) &  83.86 \\
 MM 95    & 93.14 +- (0.58) & 88.92 +- (0.29) & 95.57 +- (0.28) & 79.06 +- (2.54) & 70.27 +- (2.65) & 75.73 +- (1.95) & 86.85 +- (0.72) &  84.22 \\
 TrSc 95  & 91.86 +- (1.13) & 87.99 +- (0.30) & 95.15 +- (0.34) & 79.54 +- (1.58) & 73.37 +- (1.06) & 76.05 +- (1.23) & 87.13 +- (0.81) &  84.44 \\
 MC 95    & 93.34 +- (0.92) & 88.84 +- (0.33) & 95.69 +- (0.14) & 79.92 +- (1.32) & 71.33 +- (2.31) & 75.27 +- (1.24) & 87.08 +- (0.54) &  84.50 \\
 LC 95    & 93.29 +- (0.92) & 88.99 +- (0.23) & 95.54 +- (0.31) & 79.80 +- (1.33) & 71.40 +- (2.56) & 76.21 +- (1.49) & 86.71 +- (0.63) &  84.56 \\
 LS 95    & 93.12 +- (1.08) & 88.75 +- (0.21) & 95.56 +- (0.28) & 80.42 +- (1.35) & 71.90 +- (2.79) & 75.19 +- (1.75) & 87.00 +- (0.94) &  84.56 \\
 Evi 95   & 92.66 +- (0.63) & 88.69 +- (0.33) & 95.54 +- (0.25) & 80.75 +- (1.09) & 71.60 +- (2.14) & 76.07 +- (1.36) & 86.81 +- (1.41) &  84.59 \\
\bottomrule
\end{tabular}

==> BTW To softmax, or not to softmax that is the question (Arxiv Version) (1)/figures/merge_datasets_test_acc__baseline_roberta-base_5_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT               & IM              & CL              & S2               &   Mean \\
\midrule
 VE 95    & 91.94 +- (1.37) & 87.34 +- (0.74) & 92.84 +- (0.60) & 59.93 +- (11.72) & 56.40 +- (8.37) & 71.38 +- (0.86) & 76.73 +- (8.10)  &  76.65 \\
 Ent 95   & 93.36 +- (1.45) & 87.05 +- (1.70) & 80.17 +- (9.65) & 66.12 +- (7.31)  & 66.87 +- (4.26) & 70.30 +- (1.17) & 75.83 +- (10.07) &  77.10 \\
 KLD 95   & 82.18 +- (5.14) & 80.04 +- (4.50) & 83.49 +- (7.39) & 70.78 +- (6.51)  & 70.66 +- (3.39) & 71.75 +- (1.52) & 81.11 +- (5.05)  &  77.14 \\
 TrSc 95  & 91.23 +- (1.79) & 87.68 +- (0.82) & 94.55 +- (0.53) & 81.83 +- (2.42)  & 76.13 +- (3.72) & 71.70 +- (1.38) & 88.08 +- (3.27)  &  84.46 \\
 LS 95    & 94.76 +- (0.53) & 89.51 +- (0.39) & 95.05 +- (0.94) & 82.10 +- (2.88)  & 75.56 +- (3.12) & 74.81 +- (2.46) & 89.79 +- (2.58)  &  85.94 \\
 MC 95    & 93.74 +- (0.93) & 89.38 +- (0.58) & 94.94 +- (0.45) & 82.65 +- (1.09)  & 75.53 +- (4.47) & 75.92 +- (1.44) & 90.22 +- (0.80)  &  86.05 \\
 Evi 95   & 93.34 +- (0.61) & 89.34 +- (0.38) & 95.38 +- (0.23) & 82.55 +- (2.62)  & 77.25 +- (2.20) & 75.07 +- (1.23) & 89.72 +- (2.74)  &  86.09 \\
 TeSc 95  & 94.01 +- (0.60) & 89.70 +- (0.33) & 95.27 +- (0.43) & 82.47 +- (2.85)  & 76.67 +- (3.44) & 74.58 +- (3.52) & 91.12 +- (0.70)  &  86.26 \\
 MM 95    & 94.43 +- (0.75) & 89.75 +- (0.20) & 95.52 +- (0.54) & 82.25 +- (2.36)  & 77.82 +- (1.40) & 74.87 +- (3.53) & 90.45 +- (1.40)  &  86.44 \\
 IS 95    & 94.39 +- (0.66) & 89.53 +- (0.39) & 95.17 +- (0.31) & 82.56 +- (2.40)  & 76.57 +- (2.73) & 76.44 +- (1.37) & 90.49 +- (0.94)  &  86.45 \\
 LC 95    & 93.90 +- (1.27) & 89.40 +- (0.37) & 95.12 +- (0.42) & 83.21 +- (0.98)  & 79.02 +- (0.72) & 75.43 +- (2.11) & 90.44 +- (0.64)  &  86.65 \\
\bottomrule
\end{tabular}

==> BTW To softmax, or not to softmax that is the question (Arxiv Version) (1)/figures/merge_datasets_test_acc_clipped_baseline_bert-base-uncased_21_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT              & IM              & CL              & S2              &   Mean \\
\midrule
 KLD      & 55.53 +- (5.53) & 67.81 +- (6.19) & 88.02 +- (3.82) & 70.12 +- (2.67) & 62.01 +- (1.44) & 71.66 +- (0.91) & 77.13 +- (2.47) &  70.33 \\
 VE       & 64.68 +- (5.20) & 77.58 +- (2.57) & 93.11 +- (0.23) & 66.12 +- (8.14) & 57.64 +- (6.14) & 70.96 +- (0.63) & 75.62 +- (4.41) &  72.24 \\
 IS       & 69.99 +- (0.00) & 80.25 +- (1.07) & 93.27 +- (0.89) & 73.82 +- (1.34) & 61.67 +- (1.51) & 72.88 +- (1.61) & 78.76 +- (2.04) &  75.81 \\
 TrSc     & 69.62 +- (4.00) & 77.57 +- (1.81) & 92.99 +- (0.47) & 73.56 +- (1.87) & 67.21 +- (1.72) & 72.52 +- (1.18) & 80.74 +- (1.32) &  76.32 \\
 Evi      & 72.68 +- (2.64) & 79.42 +- (1.91) & 93.76 +- (0.39) & 74.09 +- (1.28) & 65.10 +- (2.25) & 72.80 +- (0.94) & 79.72 +- (0.72) &  76.80 \\
 TeSc     & 73.61 +- (1.32) & 79.72 +- (1.49) & 93.47 +- (0.56) & 73.58 +- (1.82) & 65.21 +- (1.08) & 72.67 +- (1.59) & 79.63 +- (0.55) &  76.84 \\
 Ent      & 72.37 +- (2.73) & 79.49 +- (1.47) & 93.80 +- (0.59) & 74.50 +- (1.62) & 65.25 +- (2.06) & 73.16 +- (0.48) & 79.94 +- (1.38) &  76.93 \\
 MC       & 73.81 +- (1.96) & 79.83 +- (1.40) & 93.45 +- (0.92) & 74.30 +- (1.38) & 64.71 +- (1.26) & 72.43 +- (1.31) & 80.20 +- (1.18) &  76.96 \\
 LC       & 75.00 +- (2.01) & 79.91 +- (1.94) & 93.81 +- (0.62) & 74.57 +- (1.33) & 65.25 +- (1.91) & 73.15 +- (0.57) & 80.22 +- (1.37) &  77.42 \\
 LS       & 74.04 +- (1.65) & 79.89 +- (1.53) & 93.63 +- (0.51) & 74.80 +- (1.38) & 65.39 +- (1.14) & 73.06 +- (0.78) & 81.35 +- (1.21) &  77.45 \\
 MM       & 75.89 +- (2.00) & 82.72 +- (0.61) & 93.80 +- (0.59) & 74.50 +- (1.62) & 65.25 +- (2.06) & 73.16 +- (0.48) & 79.94 +- (1.38) &  77.89 \\
 Rand     & 76.70 +- (2.21) & 82.22 +- (0.90) & 93.40 +- (0.34) & 75.42 +- (0.68) & 66.76 +- (2.27) & nan             & nan             &  78.90 \\
 Pass     & 96.64 +- (0.46) & 94.28 +- (0.25) & 96.66 +- (0.31) & 84.62 +- (0.46) & 82.53 +- (0.74) & nan             & nan             &  90.95 \\
\bottomrule
\end{tabular}

==> BTW To softmax, or not to softmax that is the question (Arxiv Version) (1)/figures/merge_datasets_test_acc_clipped_baseline_bert-base-uncased_5_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT               & IM              & CL              & S2              &   Mean \\
\midrule
 KLD      & 72.61 +- (9.57) & 74.27 +- (5.85) & 87.37 +- (9.89) & 76.45 +- (2.35)  & 66.20 +- (4.69) & 73.46 +- (1.93) & 81.21 +- (4.24) &  75.94 \\
 VE       & 88.46 +- (2.50) & 86.61 +- (1.95) & 94.31 +- (0.39) & 69.29 +- (10.09) & 60.78 +- (9.08) & 71.75 +- (0.97) & 81.45 +- (2.86) &  78.95 \\
 IS       & 92.10 +- (0.48) & 87.72 +- (0.40) & 95.53 +- (0.38) & 79.62 +- (1.47)  & 67.57 +- (3.22) & 76.52 +- (0.72) & 86.40 +- (1.42) &  83.64 \\
 Ent      & 91.22 +- (1.40) & 87.13 +- (0.89) & 95.57 +- (0.30) & 80.34 +- (0.97)  & 71.10 +- (1.64) & 75.45 +- (1.60) & 85.34 +- (2.36) &  83.74 \\
 TeSc     & 92.60 +- (0.75) & 88.26 +- (0.44) & 95.39 +- (0.37) & 79.41 +- (1.12)  & 70.21 +- (3.16) & 75.08 +- (2.15) & 85.76 +- (2.09) &  83.82 \\
 MC       & 92.86 +- (0.49) & 87.83 +- (0.47) & 95.47 +- (0.36) & 79.23 +- (1.66)  & 70.76 +- (3.11) & 75.40 +- (1.18) & 86.27 +- (0.74) &  83.97 \\
 TrSc     & 88.41 +- (2.61) & 86.71 +- (1.25) & 95.11 +- (0.29) & 80.29 +- (0.87)  & 73.98 +- (1.06) & 76.54 +- (1.51) & 87.10 +- (0.94) &  84.02 \\
 Evi      & 90.85 +- (1.27) & 86.85 +- (1.02) & 95.55 +- (0.31) & 80.44 +- (1.01)  & 71.49 +- (3.19) & 76.17 +- (1.28) & 86.94 +- (0.39) &  84.04 \\
 LC       & 92.87 +- (1.08) & 87.64 +- (0.37) & 95.64 +- (0.29) & 79.71 +- (2.34)  & 71.08 +- (1.42) & 75.35 +- (1.50) & 86.10 +- (1.82) &  84.06 \\
 MM       & 92.92 +- (0.62) & 88.74 +- (0.31) & 95.57 +- (0.30) & 80.34 +- (0.97)  & 71.10 +- (1.64) & 75.45 +- (1.60) & 85.34 +- (2.36) &  84.21 \\
 LS       & 92.68 +- (0.64) & 87.15 +- (1.62) & 95.60 +- (0.21) & 79.41 +- (3.13)  & 71.85 +- (2.89) & 75.89 +- (1.17) & 87.13 +- (1.18) &  84.24 \\
 Rand     & 91.71 +- (1.12) & 88.00 +- (0.28) & 94.48 +- (0.50) & 80.64 +- (0.59)  & 73.79 +- (1.08) & 74.65 +- (1.57) & 87.18 +- (0.41) &  84.35 \\
 Pass     & 96.64 +- (0.46) & 94.28 +- (0.25) & 96.66 +- (0.31) & 84.62 +- (0.46)  & 82.53 +- (0.74) & 82.64 +- (1.54) & 90.93 +- (0.48) &  89.76 \\
\bottomrule
\end{tabular}

==> BTW To softmax, or not to softmax that is the question (Arxiv Version) (1)/figures/merge_datasets_test_acc_clipped_baseline_roberta-base_21_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT              & IM              & CL              & S2              &   Mean \\
\midrule
 VE       & 75.34 +- (2.21) & 78.85 +- (1.84) & 88.08 +- (1.58) & 57.48 +- (7.95) & 56.69 +- (7.42) & 70.70 +- (0.40) & 68.62 +- (4.70) &  70.82 \\
 KLD      & 66.20 +- (3.81) & 72.38 +- (3.69) & 81.04 +- (3.59) & 70.83 +- (2.02) & 66.11 +- (2.94) & 66.21 +- (4.49) & 73.67 +- (3.78) &  70.92 \\
 TrSc     & 73.63 +- (2.44) & 79.14 +- (1.69) & 88.58 +- (2.85) & 74.14 +- (3.50) & 70.34 +- (2.31) & 71.55 +- (1.83) & 81.50 +- (2.53) &  76.98 \\
 Evi      & 75.59 +- (2.46) & 80.78 +- (1.31) & 90.94 +- (1.20) & 74.91 +- (1.97) & 70.28 +- (1.52) & 71.38 +- (3.07) & 82.01 +- (0.00) &  77.98 \\
 LS       & 78.78 +- (2.62) & 80.15 +- (1.99) & 88.97 +- (2.17) & 75.03 +- (2.54) & 71.05 +- (1.83) & 72.13 +- (1.47) & 82.47 +- (1.16) &  78.37 \\
 Ent      & 78.44 +- (2.08) & 79.33 +- (2.44) & 89.90 +- (1.55) & 76.51 +- (1.38) & 71.55 +- (1.74) & 71.57 +- (2.48) & 83.24 +- (1.34) &  78.65 \\
 IS       & nan             & 80.45 +- (1.72) & 90.81 +- (1.73) & 75.65 +- (1.46) & 71.12 +- (1.68) & 71.67 +- (2.44) & 82.19 +- (1.50) &  78.65 \\
 TeSc     & 78.91 +- (2.03) & 81.57 +- (1.67) & 90.64 +- (1.80) & 75.08 +- (1.36) & 71.69 +- (1.06) & 71.50 +- (2.62) & 83.02 +- (0.00) &  78.92 \\
 MC       & 79.10 +- (1.80) & 80.70 +- (1.85) & 90.50 +- (0.93) & 75.86 +- (2.10) & 71.49 +- (1.80) & 72.35 +- (2.25) & 82.91 +- (2.30) &  78.99 \\
 LC       & 80.04 +- (1.72) & 81.48 +- (1.24) & 90.06 +- (1.72) & 76.26 +- (1.52) & 70.44 +- (2.48) & 72.11 +- (2.01) & 83.16 +- (1.36) &  79.08 \\
 MM       & 78.45 +- (2.63) & 82.78 +- (1.77) & 89.90 +- (1.55) & 76.51 +- (1.38) & 71.55 +- (1.74) & 71.57 +- (2.48) & 83.24 +- (1.34) &  79.14 \\
 Rand     & 78.91 +- (1.78) & 82.94 +- (1.54) & 91.02 +- (1.22) & 77.48 +- (0.67) & 73.01 +- (1.48) & nan             & nan             &  80.67 \\
 Pass     & 96.84 +- (0.65) & 94.25 +- (0.37) & 96.62 +- (0.32) & 87.31 +- (0.65) & 85.07 +- (0.30) & nan             & nan             &  92.02 \\
\bottomrule
\end{tabular}

==> BTW To softmax, or not to softmax that is the question (Arxiv Version) (1)/figures/merge_datasets_test_acc_clipped_baseline_roberta-base_5_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT               & IM              & CL              & S2              &   Mean \\
\midrule
 KLD      & 81.05 +- (3.12) & 77.85 +- (3.43) & 84.44 +- (5.57) & 74.86 +- (5.10)  & 68.47 +- (5.40) & 64.68 +- (7.30) & 78.86 +- (7.17) &  75.74 \\
 VE       & 91.62 +- (1.58) & 87.35 +- (0.78) & 93.02 +- (0.62) & 59.97 +- (11.77) & 58.95 +- (9.78) & 71.38 +- (0.86) & 73.70 +- (8.57) &  76.57 \\
 TrSc     & 89.91 +- (1.76) & 87.31 +- (2.58) & 93.86 +- (3.07) & 80.14 +- (3.30)  & 74.62 +- (3.62) & 75.41 +- (1.73) & 86.76 +- (5.99) &  84.00 \\
 LS       & 93.38 +- (0.71) & 87.52 +- (1.48) & 94.04 +- (3.08) & 81.28 +- (3.09)  & 77.13 +- (2.50) & 72.96 +- (5.16) & 87.46 +- (3.87) &  84.82 \\
 Evi      & 91.94 +- (1.53) & 88.03 +- (0.84) & 95.41 +- (0.47) & 82.20 +- (2.16)  & 76.43 +- (3.26) & 74.55 +- (3.09) & 87.26 +- (3.72) &  85.12 \\
 Rand     & 92.57 +- (1.33) & 88.22 +- (0.32) & 93.64 +- (0.78) & 82.82 +- (0.73)  & 78.28 +- (1.17) & 70.52 +- (1.35) & 89.94 +- (0.59) &  85.14 \\
 MC       & 93.81 +- (0.90) & 88.19 +- (0.84) & 94.92 +- (1.08) & 80.34 +- (5.36)  & 75.28 +- (3.81) & 73.98 +- (6.51) & 90.52 +- (0.95) &  85.29 \\
 TeSc     & 93.68 +- (0.51) & 88.78 +- (0.73) & 95.19 +- (0.51) & 81.63 +- (2.60)  & 77.00 +- (1.60) & 72.61 +- (4.03) & 88.98 +- (2.39) &  85.41 \\
 IS       & 93.42 +- (1.48) & 88.46 +- (0.49) & 95.45 +- (0.29) & 83.02 +- (1.03)  & 76.63 +- (2.54) & 75.10 +- (3.50) & 89.08 +- (3.13) &  85.88 \\
 Ent      & 93.24 +- (0.77) & 87.04 +- (1.36) & 95.08 +- (0.66) & 83.43 +- (1.93)  & 77.39 +- (2.31) & 74.72 +- (3.86) & 90.49 +- (0.81) &  85.91 \\
 LC       & 93.98 +- (0.65) & 88.67 +- (0.56) & 95.40 +- (0.28) & 82.34 +- (2.51)  & 75.65 +- (2.59) & 75.96 +- (1.49) & 89.61 +- (1.47) &  85.94 \\
 MM       & 94.03 +- (0.98) & 89.49 +- (0.34) & 95.08 +- (0.66) & 83.43 +- (1.93)  & 77.39 +- (2.31) & 74.72 +- (3.86) & 90.49 +- (0.81) &  86.38 \\
 Pass     & 96.84 +- (0.65) & 94.25 +- (0.37) & 96.62 +- (0.32) & 87.31 +- (0.65)  & 85.07 +- (0.30) & 84.74 +- (1.35) & 93.63 +- (0.96) &  91.21 \\
\bottomrule
\end{tabular}

==> figures/merge_datasets_test_acc__baseline_bert-base-uncased_5_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT              & IM              & CL              & S2              &   Mean \\
\midrule
 KLD 95   & 75.10 +- (8.74) & 76.06 +- (6.00) & 87.09 +- (5.62) & 73.30 +- (8.38) & 69.30 +- (3.09) & 71.97 +- (1.22) & 81.31 +- (5.49) &  76.30 \\
 Ent 95   & 90.89 +- (1.84) & 87.17 +- (0.98) & 86.61 +- (6.55) & 72.75 +- (5.02) & 66.27 +- (4.57) & 72.19 +- (1.06) & 73.85 +- (5.96) &  78.53 \\
 VE 95    & 89.34 +- (2.18) & 87.39 +- (0.59) & 94.10 +- (0.55) & 74.41 +- (4.48) & 57.93 +- (9.43) & 71.75 +- (0.97) & 79.39 +- (6.50) &  79.19 \\
 TeSc 95  & 92.94 +- (0.60) & 88.67 +- (0.48) & 95.41 +- (0.27) & 78.88 +- (1.59) & 69.99 +- (2.61) & 74.76 +- (2.39) & 86.11 +- (1.63) &  83.82 \\
 IS 95    & 93.31 +- (0.82) & 88.70 +- (0.33) & 95.45 +- (0.31) & 78.03 +- (3.15) & 70.48 +- (1.82) & 75.01 +- (1.93) & 86.01 +- (1.56) &  83.86 \\
 MM 95    & 93.14 +- (0.58) & 88.92 +- (0.29) & 95.57 +- (0.28) & 79.06 +- (2.54) & 70.27 +- (2.65) & 75.73 +- (1.95) & 86.85 +- (0.72) &  84.22 \\
 TrSc 95  & 91.86 +- (1.13) & 87.99 +- (0.30) & 95.15 +- (0.34) & 79.54 +- (1.58) & 73.37 +- (1.06) & 76.05 +- (1.23) & 87.13 +- (0.81) &  84.44 \\
 MC 95    & 93.34 +- (0.92) & 88.84 +- (0.33) & 95.69 +- (0.14) & 79.92 +- (1.32) & 71.33 +- (2.31) & 75.27 +- (1.24) & 87.08 +- (0.54) &  84.50 \\
 LC 95    & 93.29 +- (0.92) & 88.99 +- (0.23) & 95.54 +- (0.31) & 79.80 +- (1.33) & 71.40 +- (2.56) & 76.21 +- (1.49) & 86.71 +- (0.63) &  84.56 \\
 LS 95    & 93.12 +- (1.08) & 88.75 +- (0.21) & 95.56 +- (0.28) & 80.42 +- (1.35) & 71.90 +- (2.79) & 75.19 +- (1.75) & 87.00 +- (0.94) &  84.56 \\
 Evi 95   & 92.66 +- (0.63) & 88.69 +- (0.33) & 95.54 +- (0.25) & 80.75 +- (1.09) & 71.60 +- (2.14) & 76.07 +- (1.36) & 86.81 +- (1.41) &  84.59 \\
\bottomrule
\end{tabular}

==> figures/merge_datasets_test_acc__baseline_roberta-base_5_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT               & IM              & CL              & S2               &   Mean \\
\midrule
 VE 95    & 91.94 +- (1.37) & 87.34 +- (0.74) & 92.84 +- (0.60) & 59.93 +- (11.72) & 56.40 +- (8.37) & 71.38 +- (0.86) & 76.73 +- (8.10)  &  76.65 \\
 Ent 95   & 93.36 +- (1.45) & 87.05 +- (1.70) & 80.17 +- (9.65) & 66.12 +- (7.31)  & 66.87 +- (4.26) & 70.30 +- (1.17) & 75.83 +- (10.07) &  77.10 \\
 KLD 95   & 82.18 +- (5.14) & 80.04 +- (4.50) & 83.49 +- (7.39) & 70.78 +- (6.51)  & 70.66 +- (3.39) & 71.75 +- (1.52) & 81.11 +- (5.05)  &  77.14 \\
 TrSc 95  & 91.23 +- (1.79) & 87.68 +- (0.82) & 94.55 +- (0.53) & 81.83 +- (2.42)  & 76.13 +- (3.72) & 71.70 +- (1.38) & 88.08 +- (3.27)  &  84.46 \\
 LS 95    & 94.76 +- (0.53) & 89.51 +- (0.39) & 95.05 +- (0.94) & 82.10 +- (2.88)  & 75.56 +- (3.12) & 74.81 +- (2.46) & 89.79 +- (2.58)  &  85.94 \\
 MC 95    & 93.74 +- (0.93) & 89.38 +- (0.58) & 94.94 +- (0.45) & 82.65 +- (1.09)  & 75.53 +- (4.47) & 75.92 +- (1.44) & 90.22 +- (0.80)  &  86.05 \\
 Evi 95   & 93.34 +- (0.61) & 89.34 +- (0.38) & 95.38 +- (0.23) & 82.55 +- (2.62)  & 77.25 +- (2.20) & 75.07 +- (1.23) & 89.72 +- (2.74)  &  86.09 \\
 TeSc 95  & 94.01 +- (0.60) & 89.70 +- (0.33) & 95.27 +- (0.43) & 82.47 +- (2.85)  & 76.67 +- (3.44) & 74.58 +- (3.52) & 91.12 +- (0.70)  &  86.26 \\
 MM 95    & 94.43 +- (0.75) & 89.75 +- (0.20) & 95.52 +- (0.54) & 82.25 +- (2.36)  & 77.82 +- (1.40) & 74.87 +- (3.53) & 90.45 +- (1.40)  &  86.44 \\
 IS 95    & 94.39 +- (0.66) & 89.53 +- (0.39) & 95.17 +- (0.31) & 82.56 +- (2.40)  & 76.57 +- (2.73) & 76.44 +- (1.37) & 90.49 +- (0.94)  &  86.45 \\
 LC 95    & 93.90 +- (1.27) & 89.40 +- (0.37) & 95.12 +- (0.42) & 83.21 +- (0.98)  & 79.02 +- (0.72) & 75.43 +- (2.11) & 90.44 +- (0.64)  &  86.65 \\
\bottomrule
\end{tabular}

==> figures/merge_datasets_test_acc_clipped_baseline_bert-base-uncased_21_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT              & IM              & CL              & S2              &   Mean \\
\midrule
 KLD      & 55.53 +- (5.53) & 67.81 +- (6.19) & 88.02 +- (3.82) & 70.12 +- (2.67) & 62.01 +- (1.44) & 71.66 +- (0.91) & 77.13 +- (2.47) &  70.33 \\
 VE       & 64.68 +- (5.20) & 77.58 +- (2.57) & 93.11 +- (0.23) & 66.12 +- (8.14) & 57.64 +- (6.14) & 70.96 +- (0.63) & 75.62 +- (4.41) &  72.24 \\
 IS       & 69.99 +- (0.00) & 80.25 +- (1.07) & 93.27 +- (0.89) & 73.82 +- (1.34) & 61.67 +- (1.51) & 72.88 +- (1.61) & 78.76 +- (2.04) &  75.81 \\
 TrSc     & 69.62 +- (4.00) & 77.57 +- (1.81) & 92.99 +- (0.47) & 73.56 +- (1.87) & 67.21 +- (1.72) & 72.52 +- (1.18) & 80.74 +- (1.32) &  76.32 \\
 Evi      & 72.68 +- (2.64) & 79.42 +- (1.91) & 93.76 +- (0.39) & 74.09 +- (1.28) & 65.10 +- (2.25) & 72.80 +- (0.94) & 79.72 +- (0.72) &  76.80 \\
 TeSc     & 73.61 +- (1.32) & 79.72 +- (1.49) & 93.47 +- (0.56) & 73.58 +- (1.82) & 65.21 +- (1.08) & 72.67 +- (1.59) & 79.63 +- (0.55) &  76.84 \\
 Ent      & 72.37 +- (2.73) & 79.49 +- (1.47) & 93.80 +- (0.59) & 74.50 +- (1.62) & 65.25 +- (2.06) & 73.16 +- (0.48) & 79.94 +- (1.38) &  76.93 \\
 MC       & 73.81 +- (1.96) & 79.83 +- (1.40) & 93.45 +- (0.92) & 74.30 +- (1.38) & 64.71 +- (1.26) & 72.43 +- (1.31) & 80.20 +- (1.18) &  76.96 \\
 LC       & 75.00 +- (2.01) & 79.91 +- (1.94) & 93.81 +- (0.62) & 74.57 +- (1.33) & 65.25 +- (1.91) & 73.15 +- (0.57) & 80.22 +- (1.37) &  77.42 \\
 LS       & 74.04 +- (1.65) & 79.89 +- (1.53) & 93.63 +- (0.51) & 74.80 +- (1.38) & 65.39 +- (1.14) & 73.06 +- (0.78) & 81.35 +- (1.21) &  77.45 \\
 MM       & 75.89 +- (2.00) & 82.72 +- (0.61) & 93.80 +- (0.59) & 74.50 +- (1.62) & 65.25 +- (2.06) & 73.16 +- (0.48) & 79.94 +- (1.38) &  77.89 \\
 Rand     & 76.70 +- (2.21) & 82.22 +- (0.90) & 93.40 +- (0.34) & 75.42 +- (0.68) & 66.76 +- (2.27) & nan             & nan             &  78.90 \\
 Pass     & 96.64 +- (0.46) & 94.28 +- (0.25) & 96.66 +- (0.31) & 84.62 +- (0.46) & 82.53 +- (0.74) & nan             & nan             &  90.95 \\
\bottomrule
\end{tabular}

==> figures/merge_datasets_test_acc_clipped_baseline_bert-base-uncased_5_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT               & IM              & CL              & S2              &   Mean \\
\midrule
 KLD      & 72.61 +- (9.57) & 74.27 +- (5.85) & 87.37 +- (9.89) & 76.45 +- (2.35)  & 66.20 +- (4.69) & 73.46 +- (1.93) & 81.21 +- (4.24) &  75.94 \\
 VE       & 88.46 +- (2.50) & 86.61 +- (1.95) & 94.31 +- (0.39) & 69.29 +- (10.09) & 60.78 +- (9.08) & 71.75 +- (0.97) & 81.45 +- (2.86) &  78.95 \\
 IS       & 92.10 +- (0.48) & 87.72 +- (0.40) & 95.53 +- (0.38) & 79.62 +- (1.47)  & 67.57 +- (3.22) & 76.52 +- (0.72) & 86.40 +- (1.42) &  83.64 \\
 Ent      & 91.22 +- (1.40) & 87.13 +- (0.89) & 95.57 +- (0.30) & 80.34 +- (0.97)  & 71.10 +- (1.64) & 75.45 +- (1.60) & 85.34 +- (2.36) &  83.74 \\
 TeSc     & 92.60 +- (0.75) & 88.26 +- (0.44) & 95.39 +- (0.37) & 79.41 +- (1.12)  & 70.21 +- (3.16) & 75.08 +- (2.15) & 85.76 +- (2.09) &  83.82 \\
 MC       & 92.86 +- (0.49) & 87.83 +- (0.47) & 95.47 +- (0.36) & 79.23 +- (1.66)  & 70.76 +- (3.11) & 75.40 +- (1.18) & 86.27 +- (0.74) &  83.97 \\
 TrSc     & 88.41 +- (2.61) & 86.71 +- (1.25) & 95.11 +- (0.29) & 80.29 +- (0.87)  & 73.98 +- (1.06) & 76.54 +- (1.51) & 87.10 +- (0.94) &  84.02 \\
 Evi      & 90.85 +- (1.27) & 86.85 +- (1.02) & 95.55 +- (0.31) & 80.44 +- (1.01)  & 71.49 +- (3.19) & 76.17 +- (1.28) & 86.94 +- (0.39) &  84.04 \\
 LC       & 92.87 +- (1.08) & 87.64 +- (0.37) & 95.64 +- (0.29) & 79.71 +- (2.34)  & 71.08 +- (1.42) & 75.35 +- (1.50) & 86.10 +- (1.82) &  84.06 \\
 MM       & 92.92 +- (0.62) & 88.74 +- (0.31) & 95.57 +- (0.30) & 80.34 +- (0.97)  & 71.10 +- (1.64) & 75.45 +- (1.60) & 85.34 +- (2.36) &  84.21 \\
 LS       & 92.68 +- (0.64) & 87.15 +- (1.62) & 95.60 +- (0.21) & 79.41 +- (3.13)  & 71.85 +- (2.89) & 75.89 +- (1.17) & 87.13 +- (1.18) &  84.24 \\
 Rand     & 91.71 +- (1.12) & 88.00 +- (0.28) & 94.48 +- (0.50) & 80.64 +- (0.59)  & 73.79 +- (1.08) & 74.65 +- (1.57) & 87.18 +- (0.41) &  84.35 \\
 Pass     & 96.64 +- (0.46) & 94.28 +- (0.25) & 96.66 +- (0.31) & 84.62 +- (0.46)  & 82.53 +- (0.74) & 82.64 +- (1.54) & 90.93 +- (0.48) &  89.76 \\
\bottomrule
\end{tabular}

==> figures/merge_datasets_test_acc_clipped_baseline_roberta-base_21_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT              & IM              & CL              & S2              &   Mean \\
\midrule
 VE       & 75.34 +- (2.21) & 78.85 +- (1.84) & 88.08 +- (1.58) & 57.48 +- (7.95) & 56.69 +- (7.42) & 70.70 +- (0.40) & 68.62 +- (4.70) &  70.82 \\
 KLD      & 66.20 +- (3.81) & 72.38 +- (3.69) & 81.04 +- (3.59) & 70.83 +- (2.02) & 66.11 +- (2.94) & 66.21 +- (4.49) & 73.67 +- (3.78) &  70.92 \\
 TrSc     & 73.63 +- (2.44) & 79.14 +- (1.69) & 88.58 +- (2.85) & 74.14 +- (3.50) & 70.34 +- (2.31) & 71.55 +- (1.83) & 81.50 +- (2.53) &  76.98 \\
 Evi      & 75.59 +- (2.46) & 80.78 +- (1.31) & 90.94 +- (1.20) & 74.91 +- (1.97) & 70.28 +- (1.52) & 71.38 +- (3.07) & 82.01 +- (0.00) &  77.98 \\
 LS       & 78.78 +- (2.62) & 80.15 +- (1.99) & 88.97 +- (2.17) & 75.03 +- (2.54) & 71.05 +- (1.83) & 72.13 +- (1.47) & 82.47 +- (1.16) &  78.37 \\
 Ent      & 78.44 +- (2.08) & 79.33 +- (2.44) & 89.90 +- (1.55) & 76.51 +- (1.38) & 71.55 +- (1.74) & 71.57 +- (2.48) & 83.24 +- (1.34) &  78.65 \\
 IS       & nan             & 80.45 +- (1.72) & 90.81 +- (1.73) & 75.65 +- (1.46) & 71.12 +- (1.68) & 71.67 +- (2.44) & 82.19 +- (1.50) &  78.65 \\
 TeSc     & 78.91 +- (2.03) & 81.57 +- (1.67) & 90.64 +- (1.80) & 75.08 +- (1.36) & 71.69 +- (1.06) & 71.50 +- (2.62) & 83.02 +- (0.00) &  78.92 \\
 MC       & 79.10 +- (1.80) & 80.70 +- (1.85) & 90.50 +- (0.93) & 75.86 +- (2.10) & 71.49 +- (1.80) & 72.35 +- (2.25) & 82.91 +- (2.30) &  78.99 \\
 LC       & 80.04 +- (1.72) & 81.48 +- (1.24) & 90.06 +- (1.72) & 76.26 +- (1.52) & 70.44 +- (2.48) & 72.11 +- (2.01) & 83.16 +- (1.36) &  79.08 \\
 MM       & 78.45 +- (2.63) & 82.78 +- (1.77) & 89.90 +- (1.55) & 76.51 +- (1.38) & 71.55 +- (1.74) & 71.57 +- (2.48) & 83.24 +- (1.34) &  79.14 \\
 Rand     & 78.91 +- (1.78) & 82.94 +- (1.54) & 91.02 +- (1.22) & 77.48 +- (0.67) & 73.01 +- (1.48) & nan             & nan             &  80.67 \\
 Pass     & 96.84 +- (0.65) & 94.25 +- (0.37) & 96.62 +- (0.32) & 87.31 +- (0.65) & 85.07 +- (0.30) & nan             & nan             &  92.02 \\
\bottomrule
\end{tabular}

==> figures/merge_datasets_test_acc_clipped_baseline_roberta-base_5_25_25_20.tex <==
\begin{tabular}{llllllllr}
\toprule
 Method   & TR              & AG              & SU              & RT               & IM              & CL              & S2              &   Mean \\
\midrule
 KLD      & 81.05 +- (3.12) & 77.85 +- (3.43) & 84.44 +- (5.57) & 74.86 +- (5.10)  & 68.47 +- (5.40) & 64.68 +- (7.30) & 78.86 +- (7.17) &  75.74 \\
 VE       & 91.62 +- (1.58) & 87.35 +- (0.78) & 93.02 +- (0.62) & 59.97 +- (11.77) & 58.95 +- (9.78) & 71.38 +- (0.86) & 73.70 +- (8.57) &  76.57 \\
 TrSc     & 89.91 +- (1.76) & 87.31 +- (2.58) & 93.86 +- (3.07) & 80.14 +- (3.30)  & 74.62 +- (3.62) & 75.41 +- (1.73) & 86.76 +- (5.99) &  84.00 \\
 LS       & 93.38 +- (0.71) & 87.52 +- (1.48) & 94.04 +- (3.08) & 81.28 +- (3.09)  & 77.13 +- (2.50) & 72.96 +- (5.16) & 87.46 +- (3.87) &  84.82 \\
 Evi      & 91.94 +- (1.53) & 88.03 +- (0.84) & 95.41 +- (0.47) & 82.20 +- (2.16)  & 76.43 +- (3.26) & 74.55 +- (3.09) & 87.26 +- (3.72) &  85.12 \\
 Rand     & 92.57 +- (1.33) & 88.22 +- (0.32) & 93.64 +- (0.78) & 82.82 +- (0.73)  & 78.28 +- (1.17) & 70.52 +- (1.35) & 89.94 +- (0.59) &  85.14 \\
 MC       & 93.81 +- (0.90) & 88.19 +- (0.84) & 94.92 +- (1.08) & 80.34 +- (5.36)  & 75.28 +- (3.81) & 73.98 +- (6.51) & 90.52 +- (0.95) &  85.29 \\
 TeSc     & 93.68 +- (0.51) & 88.78 +- (0.73) & 95.19 +- (0.51) & 81.63 +- (2.60)  & 77.00 +- (1.60) & 72.61 +- (4.03) & 88.98 +- (2.39) &  85.41 \\
 IS       & 93.42 +- (1.48) & 88.46 +- (0.49) & 95.45 +- (0.29) & 83.02 +- (1.03)  & 76.63 +- (2.54) & 75.10 +- (3.50) & 89.08 +- (3.13) &  85.88 \\
 Ent      & 93.24 +- (0.77) & 87.04 +- (1.36) & 95.08 +- (0.66) & 83.43 +- (1.93)  & 77.39 +- (2.31) & 74.72 +- (3.86) & 90.49 +- (0.81) &  85.91 \\
 LC       & 93.98 +- (0.65) & 88.67 +- (0.56) & 95.40 +- (0.28) & 82.34 +- (2.51)  & 75.65 +- (2.59) & 75.96 +- (1.49) & 89.61 +- (1.47) &  85.94 \\
 MM       & 94.03 +- (0.98) & 89.49 +- (0.34) & 95.08 +- (0.66) & 83.43 +- (1.93)  & 77.39 +- (2.31) & 74.72 +- (3.86) & 90.49 +- (0.81) &  86.38 \\
 Pass     & 96.84 +- (0.65) & 94.25 +- (0.37) & 96.62 +- (0.32) & 87.31 +- (0.65)  & 85.07 +- (0.30) & 84.74 +- (1.35) & 93.63 +- (0.96) &  91.21 \\
\bottomrule
\end{tabular}
